4DAC: Learning Attribute Compression for Dynamic Point Clouds

With the development of the 3D data acquisition facilities, the increasing scale of acquired 3D point clouds poses a challenge to the existing data compression techniques. Although promising performance has been achieved in static point cloud compression, it remains under-explored and challenging to leverage temporal correlations within a point cloud sequence for effective dynamic point cloud compression. In this paper, we study the attribute (e.g., color) compression of dynamic point clouds and present a learning-based framework, termed 4DAC. To reduce temporal redundancy within data, we first build the 3D motion estimation and motion compensation modules with deep neural networks. Then, the attribute residuals produced by the motion compensation component are encoded by the region adaptive hierarchical transform into residual coefficients. In addition, we also propose a deep conditional entropy model to estimate the probability distribution of the transformed coefficients, by incorporating temporal context from consecutive point clouds and the motion estimation/compensation modules. Finally, the data stream is losslessly entropy coded with the predicted distribution. Extensive experiments on several public datasets demonstrate the superior compression performance of the proposed approach.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   \country is now obligatory for addresses.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> chapters/name.tex <==

\begin{figure*}[t]
	\centering
	\includegraphics[width=1.0\linewidth]{Figures/040_Experiments/paper_quant.pdf}
	
    \caption{Quantitative results}
	\label{fig:exp_qual_scannet}
\end{figure*}


\begin{figure}[t]
	\begin{center}
    	\includegraphics[width=1.0\linewidth]{sample/Figures/040_Experiments/exp_downstream.pdf}
	\end{center}
    \caption{The quantitative results for two downstream tasks. 
    }
	\label{fig:scannet_seg}
\end{figure}



% \begin{figure*}[t]
% 	\centering
% 	\includegraphics[width=1.0\linewidth]{sample/Figures/appendix_quant_gpcc.pdf}
	

% \begin{figure*}[t]
% 	\centering
% 	\includegraphics[width=1.0\linewidth]{sample/Figures/appendix_quant_dl.pdf}
	
	





==> chapters/temp.tex <==


\section{Additional Method Details}




\begin{figure}[t]
	\centering
	\includegraphics[width=1.0\linewidth]{Figures/070_Appendix/memc.pdf}
    \caption{The proposed Motion Estimation Net (a) and Motion Compensation Net (b).
    }
	\label{fig:memc}
\end{figure}



\subsection{Motion Estimation and Compensation}

The motion estimation network and the motion compensation network are shown in Fig. \ref{fig:memc}. We construct our motion estimation and motion compensation nets with modules (\emph{Set Conv}, \emph{Flow Embedding} and \emph{Set Upconv}) proposed by FlowNet3D \cite{liu2019flownet3d}. Our \emph{Attribute Embedding} shares the same structure with the \emph{Flow Embedding}. Because the motion compensation net extracts point cloud attribute information rather than motion information, we denote this feature fusion module as \emph{Attribute Embedding} in Fig. \ref{fig:memc}(b). 











\subsection{Transform Coding}\label{sec:Transform Coding appendix}



In this paper, we use Region Adaptive Hierarchical Transform (RAHT) \cite{de2016compression} for transform coding. In the following parts, we first introduce RAHT, and then show how to construct a RAHT tree.


Different from the common 2D wavelet transform, RAHT processes empty spaces through transmitting low-frequency coefficients to the next depth level directly when the point has no neighbor. 



\subsubsection{Region Adaptive Hierarchical Transform}\label{sec:Region Adaptive Hierarchical Transform appendix}



RAHT transforms point cloud attributes to frequency-domain coefficients based on 3D Haar wavelet transform. Specifically, the algorithm takes a voxelized point cloud as input, and convert attributes to low- and high-frequency coefficients along three dimensions repeatedly. Different from the common 2D wavelet transform, RAHT is able to process empty spaces through transmitting low-frequency coefficients to the next depth level directly when the point has no neighbor. Another difference is that the wavelet basis is adaptive to the number of points in the corresponding region. More specifically, two low-frequency neighbors are decomposed to low- and high-frequency coefficients following:
\begin{equation}
\left[\begin{array}{c}
l_{d+1, x, y, z} \\
h_{d+1, x, y, z}
\end{array}\right]=\frac{1}{\sqrt{w_{1}+w_{2}}}\left[\begin{array}{cc}
\sqrt{w_{1}} & \sqrt{w_{2}} \\
-\sqrt{w_{2}} & \sqrt{w_{1}}
\end{array}\right]\left[\begin{array}{c}
l_{d, 2 x, y, z} \\
l_{d, 2 x+1, y, z}
\end{array}\right],
\end{equation}
where $l_{d, 2 x, y, z}$ and $l_{d, 2 x+1, y, z}$ are two low-frequency neighbors along the $x$ dimension, and $w_{1}$ and $w_{2}$ are their weights (\textit{i.e.}, the number of points in the corresponding subspace). $l_{d+1, x, y, z}$ and $h_{d+1, x, y, z}$ are the decomposed low- and high-frequency coefficients, respectively. 





% \begin{equation}
% \left[\begin{array}{l}
% l_{d+1, x, y, z} \\
% h_{d+1, x, y, z}
% \end{array}\right]=\mathbf{T}_{w_{1}, w_{2}}\left[\begin{array}{c}
% l_{d, 2 x, y, z} \\
% l_{d, 2 x+1, y, z}
% \end{array}\right]\label{con:raht},
% \end{equation}
% where $l_{d, 2 x, y, z}$ and $l_{d, 2 x+1, y, z}$ are two low-frequency neighbors along the $x$ dimension, and $l_{d+1, x, y, z}$ and $h_{d+1, x, y, z}$ are the decomposed low- and high-frequency coefficients, respectively. Here, $\mathbf{T}_{w_{1}}$ is defined as
% \begin{equation}
% \mathbf{T}_{w_{1}, w_{2}}=\frac{1}{\sqrt{w_{1}+w_{2}}}\left[\begin{array}{cc}
% \sqrt{w_{1}} & \sqrt{w_{2}} \\
% -\sqrt{w_{2}} & \sqrt{w_{1}}
% \end{array}\right],
% \end{equation}
% where $w_{1}$ and $w_{2}$ are the weights (\textit{i.e.}, the number of points in the corresponding subspace) of $l_{d, 2x, y, z}$ and $l_{d, 2x+1, y, z}$, respectively. 








\subsubsection{RAHT Tree}\label{sec:RAHT Tree appendix}



We revisit the transform process of RAHT and the construction of a RAHT tree through a 2D toy example in Fig. \ref{fig:method_raht} \cite{3dac}. Low- and high-frequency coefficients, $l_{i}$ and $h_{i}$, is represented as green and yellow blocks, respectively. During encoding, transform is conducted along the $x$ axis and then the $y$ axis repeatedly until all voxelized points are merged. At the first depth level, along the $x$ axis, points without neighbor (\textit{i.e.}, $l_{1}$), are transmitted to the next depth level and those with a neighbor (\textit{i.e.}, $l_{2}$ and $l_{3}$) are decomposed to low- and high-frequency coefficients (\textit{i.e.}, $l_{4}$ and $h_{1}$). In this way, we transform low-frequency coefficients depth by depth until generating the DC coefficient $l_{5}$. After forward transform, we compress and transmit the DC coefficient and all high-frequency coefficients, and thus we can decode all low-frequency coefficients from the root depth level to the leaf level. Specifically, decoding is start from the root level through reconverting the DC coefficient $l_{5}$ and high-frequency coefficient $h_{2}$ to low-frequency coefficients of the previous depth (\textit{i.e.}, $l_{1}$ and $l_{4}$). In this way, all low-frequency coefficients can be regenerated depth by depth.


Here, we further construct the RAHT tree of the aforementioned toy example for temporal context feature extraction in Sec. \ref{sec:Entropy Model}. Following the hierarchical transform processes, the RAHT tree is constructed as Fig. \ref{fig:method_raht}(b). Low-frequency coefficients of the first depth level (\textit{i.e.}, point cloud attributes), $l_{1}$, $l_{1}$ and $l_{3}$, are set as leaf nodes. These tree nodes are transmitted or merged according to the repeated transform steps. For example,
tree nodes of $l_{2}$ and $l_{3}$ are merged to that of $l_{4}$ and $h_{1}$, while tree node of $l_{1}$ is sent to the next depth level. Thanks to the hierarchical structure, this RAHT tree is available for not only intra-tree spatial feature extraction \cite{3dac} but also inter-tree temporal feature aggregation between two consecutive point clouds in Sec. \ref{sec:Entropy Model}. 



\section{Additional Architecture Details}


\subsection{Architecture Details}



\subsection{Implementation Details}


For faster convergence when training these networks, we multiply the output vectors of the motion estimation net with learnable tensors which are initialized as zeros, and use the result as the estimated motion vectors $V^{(t)}$.






\section{Additional Experiments}

\subsection{Comparison with G-PCC}


\subsection{Comparison with Learning-based Methods}


\subsection{Run Time}





\section{Additional Qualitative Results}




\begin{figure}[t]
	\centering
	\includegraphics[width=1.0\linewidth]{Figures/070_Appendix/method_raht_3dac.pdf}
    \caption{raht. 
    }
	\label{fig:scannet_seg}
\end{figure}




\begin{figure*}[t]
	\centering
	\includegraphics[width=1.0\linewidth]{Figures/070_Appendix/appendix_quant_gpcc.pdf}
    \caption{The quantitative results compared with gpcc-based methods. 
    }
	\label{fig:scannet_seg}
\end{figure*}

\begin{figure*}[t]
	\centering
	\includegraphics[width=1.0\linewidth]{Figures/070_Appendix/appendix_quant_dl.pdf}
    \caption{The quantitative results compared with learning-based methods. 
    }
    \label{fig:scannet_seg}
\end{figure*}	




